CLIO: a Novel Robotic Solution for Exploration and Rescue Missions in Hostile Mountain Environments

Rescue missions in mountain environments are hardly achievable by standard legged robots-because of the high slopes-or by flying robots-because of limited payload capacity. We present a concept for a rope-aided climbing robot which can negotiate up-to-vertical slopes and carry heavy payloads. The robot is attached to the mountain through a rope, and it is equipped with a leg to push against the mountain and initiate jumping maneuvers. Between jumps, a hoist is used to wind/unwind the rope to move vertically and affect the lateral motion. This simple (yet effective) two-fold actuation allows the system to achieve high safety and energy efficiency. Indeed, the rope prevents the robot from falling while compensating for most of its weight, drastically reducing the effort required by the leg actuator. We also present an optimal control strategy to generate point-to-point trajectories overcoming an obstacle. We achieve fast computation time (<1 s) thanks to the use of a custom simplified robot model. We validated the generated optimal movements in Gazebo simulations with a complete robot model with a < 5% error on a 16 m long jump, showing the effectiveness of the proposed approach, and confirming the interest of our concept. Finally, we performed a reachability analysis showing that the region of achievable targets is strongly affected by the friction properties of the foot-wall contact.

==> sections/control.tex <==
As anticipated in the system description above, one of the most
complex aspects of this system is that part of the control, the
$\vect{F}_u$ force, has an impulsive nature.  Its effect can be
modeled as an instantaneous reset of the velocities $\dot{\theta}$ and
$\dot{\phi}$, i.e., $x_4$ and $x_5$, respectively.  More precisely,
this effect is modelled using known state-of-the-art
results~\cite{dim17}, i.e.
\begin{equation}
  \label{eq:Reset}
  \begin{aligned}
    &x_4(t_0^+) = x_4(t_0^-) + \frac{1}{m x_3(t_0^-)} F_{u,n},\\
    &x_5(t_0^+) = x_5(t_0^-) +  \frac{1}{m x_3(0) \sin x_1(0)} F_{u,t} .
  \end{aligned}
\end{equation}
Due to the imprecisions in the actuators and to the lack of knowledge
on the terrain characteristics, the velocities after the reset could
differ from the expected values hence perturbing the whole trajectory.
The only possibility for fixing the deviation is to rely on the only
control variable available during the flight, i.e., the traction force
$F_r$, and use it within a feedback control law.  In this
section, we first address the controllability problem, i.e., if
such a feedback law can be found for an under-actuated system like ours. 
Second, we show how to design such a feedback control law.

%\subsection{Local Reachability}
%
%Let us consider the system canonical form~\eqref{eq:NonLinStateSpace},
%with the availability of the input $F_r$, while
%$F_{u,n} = F_{u,t} = 0$ assuming resets and impulsive forces as
%in~\eqref{eq:Reset}. By recalling the results
%in~\cite{isidori1985nonlinear}, we can compute the involutive
%distribution $\Delta_n(\vect{x})$ and conclude for local reachability
%iff $\Delta_n(\vect{x})$ is nonsingular. As such, consider the system
%state $\vect{x}$ and the dynamic in~\eqref{eq:NonLinStateSpace},
%rewritten as
%\begin{equation}
%  \label{eq:VecFields}
%  \dot {\vect{x}} = f(\vect{x}) + g_r(\vect{x}) F_{r} ,
%\end{equation}
%hence the initial distribution is given by the column
%\[
%  \Delta_0(\vect{x}) = \{g_r(\vect{x})\} .
%\]
%It is then possible to derive
%\[
%  \Delta_1(\vect{x}) = \{\Delta_0(\vect{x}),
%  [f(\vect{x}),g_r(\vect{x})]\} = \{\Delta_0(\vect{x}), [f(\vect{x}),
%  \Delta_0(\vect{x})]\} ,
%\]
%where $[\cdot,\cdot]$ are the usual Lie bracket
%operators~\cite{isidori1985nonlinear}, i.e.
%\[
%  [f(\vect{x}),g_r(\vect{x})] = \frac{\partial g_r(\vect{x})}{\partial
%    \vect{x}}f(\vect{x}) - \frac{\partial f(\vect{x})}{\partial
%    \vect{x}}g_r(\vect{x}) .
%\]
%It is then possible to derive in a recursive manner
%\[
%  \Delta_{n+1}(\vect{x}) = \{\Delta_n(\vect{x}),
%  [f(\vect{x}),\Delta_n(\vect{x})]\} ,
%\]
%where, with a slight abuse of notation,
%$[f(\vect{x}),\Delta_n(\vect{x})]$ is intended as the Lie brackets of
%$f(\vect{x})$ with respect to all the vector fields of
%$\Delta_n(\vect{x})$. After carrying out all the computations, it turns out that
%$\dim\{\mbox{span}\{\Delta_5\}\} = 6$, i.e., the distribution is
%nonsingular and, hence, the system is locally reachable.
%
%\subsection{Lyapunov-based control design}
%
%One possible path to design a state-feedback, Lyapunov-based
%controller for the system~\eqref{eq:NonLinStateSpace} is to use the
%backstepping technique~\cite{krstic1995nonlinear}. Let us define the
%following Lyapunov function candidate on the position subsystem
%\[
%  V_1(x_1, x_2, x_3) = \frac{1}{2} [(x_1 - \overline x_1)^2 +
%  (x_2 - \overline x_2)^2 + (x_3 - \overline x_3)^2] ,
%\]
%where the quantities $\overline \cdot$ are the desired, final values
%and whose time derivative is simply given by
%\[
%  \dot V_1(x_1, x_2, l) = (x_1 - \overline x_1) x_4 +
%  (x_2 - \overline x_2) x_5 + (x_3 - \overline x_3) x_6 . 
%\]
%Hence, assuming the proportional control laws (with
%$k_{x_1}, k_{x_2}, k_{x_3} > 0$)
%\begin{equation}
%  \label{eq:LyapBack}
%    x_4 = - k_{x_1}  (x_1 - \overline x_1), 
%    x_5 = - k_{x_2}  (x_2 - \overline x_2), 
%    x_6 = - k_{x_3} (x_3 - \overline x_3),
%\end{equation}
%we have immediately that
%$[\overline x_1, \overline x_2, \overline x_3]^T$ is an asymptotically
%stable equilibrium point for the subsystem. When the entire state
%$\vect{x}$ is considered, the quantities in~\eqref{eq:LyapBack} are
%treated as desired and then define the following Lyapunov function
%candidate
%\[
%  V(\vect{x}) = V_1(x_1, x_2, x_3) + \frac{1}{2} [(x_4 - \overline
%  x_4)^2 + (x_5 + \overline x_5)^2 + (x_6 + \overline x_6)^2] .
%\]
%The time derivative becomes
%\[
%  \begin{aligned}
%    \dot V(\vect{x}) = &(x_4 - \overline x_4) (f_4(\vect{x}) -
%    \dot{\overline x}_4) + (x_5 - \overline x_5)
%    (f_5(\vect{x}) - \dot{\overline x}_5) + \\
%    & + (x_6 - \overline x_6) \left (f_6(\vect{x}) + \frac{F_{r}}{m} -
%      \dot{\overline x}_6 \right ) + \dot V_1(x_1, x_2, x_3),
%  \end{aligned}
%\]
%where $f_i(\vect{x})$ is the $i$-th vector of the vector field
%$f(\vect{x})$ in~\eqref{eq:VecFields} and where we have
%from~\eqref{eq:LyapBack}
%\[
%  \begin{aligned}
%    \dot{\overline x_4} & = - k_{x_1}  x_4 , \\
%    \dot{\overline x_5} & = - k_{x_2} x_5 , \\
%    \dot{\overline x_6} & = - k_{x_3} r . 
%  \end{aligned}
%\]
%It is therefore immediate to notice that the Lyapunov candidate time
%derivative $\dot V(x)$ is negative definite with the following control
%laws (with $k_{x_4}, k_{x_5}, k_{x_6} > 0$)
%\[
%  \begin{aligned}
%    F_{u,n} & = -ml (f_4(x) + k_{x_4} (x_4 - \overline x_4) + k_{x_1}  x_4) , \\
%    F_{u,t} & = -ml s_{x_1} (f_5(x) + k_{x_5} (x_5 - \overline x_5) + k_{x_5}  x_5) , \\
%    F_{r} & = -m (f_6(x) + k_{x_6} (r - \overline x_6) + k_{x_3} r) , \\
%  \end{aligned}
%\]
%thus proving the asymptotic stability of the equilibrium
%$[\overline x_1, \overline x_2, \overline x_3, 0, 0, 0]^T$ for the
%system~\eqref{eq:CanonicalForm}.
%
%In a more realistic case, we can assume that $F_{u,n} = F_{u,t} = 0$
%right after the application of the impulsive inputs, thus we will
%study how a stabilising Lyapunov-based control law can be designed
%using only the input $F_{x_6}$. To this end, we first prove that the
%system remains locally reachable. To this end, we define the reduced
%version of~\eqref{eq:VecFields} as
%\[
%  \dot x = f(x) + g_{x_6}(x) F_{r} ,
%\]
%where the effect of the impulsive forces is supposed to be stored in
%the state $x$ right after their applications. Hence, the initial
%distribution is
%\[
%  \Delta_0 = \{g_{x_6}\} .
%\]
%It is then possible to derive in a recursive way
%\[
%  \Delta_{n+1} = \{\Delta_n, [f,\Delta_n]\} .
%\]
%It turns then out that $\mbox{span}\Delta_5 = 6$, i.e., the
%distribution is nonsingular and, hence, the system is locally
%reachable.
%
%In this case, we assume that a reference trajectory for the angles
%$x_1$ and $x_2$ is given, for example given by the first two
%of~\eqref{eq:LyapBack}, for which both the first and second derivative
%can be computed. We can then consider the following Lyapunov candidate
%\[
%  V(x) = \frac{1}{2} [(x_1 - \overline x_1)^2 + (x_2 -
%  \overline x_2)^2 + (l - \overline x_3)^2 + (x_4 -
%  \overline x_4)^2 + (x_5 + \overline x_5)^2 + r^2] ,
%\]
%whose time derivative is given by
%\[
%  \dot V(x) = (x_1 - \overline x_1) x_4 + (x_2 -
%  \overline x_2) x_5 + (l - \overline x_3) r + h_1(x_4) + h_2(x_5)
%  + r (f_6(x) + \frac{F_{r}}{m}),
%\]
%where
%\[
%  \begin{aligned}
%    h_1(x_4) = & (x_4 - \overline x_4) (f_4(x) -
%    \dot{\overline x_4}) , \\
%    h_2(x_5) = & (x_5 - \overline x_5) (f_5(x) -
%    \dot{\overline x_5}) . \\    
%  \end{aligned}
%\]
%We can then build a Lyapunov control law that locally controls the
%system dynamics.


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../icra22climb"
%%% End:

